On the diagonal hooks of a symmetric partition

Using only a symmetric p-core partition and p-quotient, we give an explicit formula for the set of diagonal hook lengths of the associated symmetric partition.

==> On_diagonal_hooks_arxiv_figures.tex <==
\begin{figure}[h!]
\caption{Removing a single $p$-hook}
\[\begin{xy}<1cm,0cm>:
(-1,0)*+!D{x'}*+{\circ}; (1,0)*+!D{x}*+{\bullet}
**\crv{(0,-1)}?<*\dir{<};
(0,-.5);(0,1)*+{\theta(\lambda)}**\dir{-};
\end{xy}\]
\end{figure
\begin{figure}[h!]
\caption{Removing non-straddling $p$-hooks}
\[\begin{xy}<1cm,0cm>:
(-1,0)*+!D{y'}*+{\bullet}; (-3,0)*+!D{x'}*+{\circ}
**\crv{(-2,-1)}?>*\dir{>};
(0,-.5);(0,1)*+{\theta(\lambda)}**\dir{-}; (3,0)*+!D{x}*+{\bullet};
(1,0)*+!D{y}*+{\circ}
**\crv{(2,-1)}?>*\dir{>};
\end{xy}\]
\end{figure}
\begin{figure}[h!]
\caption{Removing straddling $p$-hooks}
\[\begin{xy}<1cm,0cm>:
(-1,0)*+!D{y}*+{\circ}; (3,0)*+!D{x}*+{\bullet}
**\crv{(1,-1)}?<*\dir{<};
(0,-.5);(0,1)*+{\theta(\lambda)}**\dir{-}; (-3,0)*+!D{x'}*+{\circ};
(1,0)*+!D{y'}*+{\bullet}
**\crv{(-1,-1)}?<*\dir{<};
\end{xy}\]
\end{figure}
\begin{figure}[h!]
\caption{$p$-quotient of Example 5.7}
\[\begin{xy}<1.35in,0in>:
(2,1)*+{\emptyset}="0"; (0,0)*+{\emptyset}**\dir{-};
(0,-1)*{D_0\left(\lambda\right)=\emptyset};
"0";(1,0)*+{\emptyset}**\dir{-};
(1,-.75)*{D_1\left(\lambda\right)=\emptyset};
"0";(2,0)*+!U{\yng(2,2)}**\dir{-};
(2,-1)*{D_2\left(\lambda\right)=\left\{1,0\left|1,0\right|\right\}};
"0";(3,0)*+{\emptyset}**\dir{-};
(3,-.75)*{D_3\left(\lambda\right)=\emptyset};
"0";(4,0)*+{\emptyset}**\dir{-}; (4,-1)*{D_4(\lambda)=\emptyset};
\end{xy}\]
\end{figure}

